Polyhedral Collision Detection via Vertex Enumeration

Collision detection is a critical functionality for robotics. The degree to which objects collide cannot be represented as a continuously differentiable function for any shapes other than spheres. This paper proposes a framework for handling collision detection between polyhedral shapes. We frame the signed distance between two polyhedral bodies as the optimal value of a convex optimization, and consider constraining the signed distance in a bilevel optimization problem. To avoid relying on specialized bilevel solvers, our method exploits the fact that the signed distance is the minimal point of a convex region related to the two bodies. Our method enumerates the values obtained at all extreme points of this region and lists them as constraints in the higher-level problem. We compare our formulation to existing methods in terms of reliability and speed when solved using the same mixed complementarity problem solver. We demonstrate that our approach more reliably solves difficult collision detection problems with multiple obstacles than other methods, and is faster than existing methods in some cases.

==> background.tex <==
In this paper we focus on optimization-based collision-avoidance, the main advantage of optimization-based collision avoidance is that it allows for convenient modeling of variety of objectives, constraints and dynamics using the existing nonlinear optimization frameworks. 
The solutions to this constrained trajectory optimization problem then defines feasible and (locally) optimal trajectories. In this section, we provide a brief overview of the current state of optimization-based collision-avoidance.

There are multiple ways of encoding obstacles for optimization-based collision-avoidance in a way that trajectory optimization frameworks can handle. A most common and efficient approach which does not involve the signed distance function utilizes the hyperplane separation theorem, which states there exists a separating hyperplane that separates two non-empty non-intersecting closed convex objects. 
However, this approach is less inductive to the situation when two convex polyhedra are actually intersecting each other, and it gives no information about the distance between two objects if they are not intersecting.

It is common to define some form of distance function that indicates how far two objects are intersecting each other.
In this work, we use a symmetric signed distance function that is based on the notion of inflating (or deflating) a convex polyhedron uniformly.
The signed distance function is evaluated by solving a convex optimization problem.
The signed distance as a function of problem parameters such as the ego position and orientation is in general a non-smooth function, except for simple bounding sphere approaches. 

The most straightforward approach is to directly encode the KKT conditions that correspond to the signed distance minimization problem and the geometric constraints directly into the problem.
The main limitation of this approach is that the top-level problem cannot reason about the directly embedded low-level problem of collision detection.
We later demonstrate that this method does not work well for anything but the simplest of example problems, because the low-level collision detection problem is not differentiable. 

In \cite{zhang_optimization-based_2021}, the authors propose a method based on the notion of signed distance in order to exactly reformulate the non-differentiable collision-avoidance constraints using strong duality of convex optimization.
In \cite{landry_path_2012}, the authors represent the ego and the obstacles as finite unions of convex compact polyhedra, combined with Farkas’s lemma allows them to express the collision avoidance as state constraints.
However, this approach is flawed, because when inequality constraints are weakly active at the solution of the low-level problem, the implicit function theorem cannot be evoked. 


Similarly, in \cite{tracy2023differentiable}, the authors formulate the collision detection problem using a signed distance function as a convex optimization problem with conic constraints, but in practice they ignore the non-existence of the gradient of the Lagrangian that corresponds to the conic problem of minimizing the signed distance function.
While the set of points in problem data space where the derivatives of the problem with respect to the problem data do not exist is of measure zero, we demonstrate that ignoring the non-differentiability of the signed distance function negatively impacts the reliability and performance of this approach for complex and difficult collision avoidance problems.





==> outline.tex <==
\begin{enumerate}
\item Intro
    \begin{enumerate}
        \item Collision detection is a key problem in motion planning
        \item Bounding spheres approximation is overused, can be inefficient for complex geometries
        \item Why optimization-based collision avoidance?
    \end{enumerate}
\item Related Work
    \begin{enumerate}
        \item dynamic programming, reachability analysis, graph search, random sampling, interpolating curves
        \item optimization-based approaches: point-mass (spheres) vs polytopes
    \end{enumerate}
\item Problem Definition
   \begin{enumerate}
        \item Symmetric sign distance with uniform inflation/deflation
        \item vertices, interior/exterior points
    \end{enumerate}
\item Simulations
    \begin{enumerate}
         \item We compare our problem formulation to three different problem formulations and attempt to solve exactly the same problems using PATHSolver with identical parameters.
        \item Why did we choose to compare it to this: Theory, advantages, disadvantages
        \item Separating hyperplanes, DifferentiableCollisions.jl, direct KKT
        \item  We compare our formulation and comparison baselines on the following problems: simple packing, simple gap, piano, random packing, L through gap, L packing
    \end{enumerate}
\item Other
\begin{enumerate}
    \item what to change going forward
\end{enumerate}
\end{enumerate}



